Technical Report: Optimal Control of Piecwise-smooth Control Systems via Singular Perturbations

This paper investigates optimal control problems formulated over a class of piecewise-smooth vector fields. Instead of optimizing over the discontinuous system directly, we instead formulate optimal control problems over a family of regularizations which are obtained by "smoothing out" the discontinuity in the original system. It is shown that the smooth problems can be used to obtain accurate derivative information about the non-smooth problem, under standard regularity conditions. We then indicate how the regularizations can be used to consistently approximate the non-smooth optimal control problem in the sense of Polak. The utility of these smoothing techniques is demonstrated in an in-depth example, where we utilize recently developed reduced-order modeling techniques from the dynamic walking community to generate motion plans across contact sequences for a 18-DOF model of a lower-body exoskeleton.

==> abstract.tex <==
This paper investigates optimal control problems formulated over a class of piecewise-smooth vector fields. Instead of optimizing over the discontinuous system directly, we instead formulate optimal control problems over a family of regularizations which are obtained by "smoothing out" the discontinuity in the original system. It is shown that the smooth problems can be used to obtain accurate derivative information about the non-smooth problem, under standard regularity conditions. We then indicate how the regularizations can be used to consistently approximate the non-smooth optimal control problem in the sense of Polak. The utility of these smoothing techniques is demonstrated in an in-depth example, where we utilize recently developed reduced-order modeling techniques from the dynamic walking community to generate motion plans across contact sequences for a 18-DOF model of a lower-body exoskeleton. 
